On Hydrodynamic Correlations in Low-Dimensional Interacting Systems

Low-dimensional systems are an important field of current theoretical and experimental research. Recent technological developments provide many possible realizations of effectively one-dimensional systems. These devices promise to give us access to a new range of phenomena. It is therefore very interesting to develop theoretical methods specific for such systems to model their behavior and calculate the correlators of the resulting theory. Incidentally, one such method exists and is known as Bosonization. It can be applied to one-dimensional systems and effectively describes low energy excitations in a universal way. We use the example of a correlator known as the Emptiness Formation Probability to show that Bosonization fails to describe some long range correlators corresponding to large disturbances (the EFP measures the probability for the ground state of the system to develop a region without particles). We trace this failure to the fact that Bosonization is constructed as a linear approximation of the full theory and we set up to develop a collective description with the required non-linearity. The resulting scheme is essentially a Hydrodynamic paradigm for quantum systems. We show how to construct such a hydrodynamic description for a variety of exactly integrable models and illustrate how it can be used to make new predictions. For the special case of the spin-1/2 XY model we take advantage of the structure of the model to express the EFP as a determinant of a very special type of matrix, known as Toeplitz Matrix. We use the theory of Toeplitz determinants to calculate the asymptotic behavior of the EFP in the XY model and discuss its relation with the criticality of the theory.

==> Chap6-LatticeHydro.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Free fermions on the lattice}
\label{sec_lattice}

The goal of this section is to illustrate that the hydrodynamic method we used is not limited to Galilean invariant systems. We use the method to calculate the EFP for a system of non-interacting lattice fermions with an arbitrary dispersion $\varepsilon(k)$.
Semiclassically, one can describe the evolution of the degenerate 1D Fermi gas in terms of two smooth and slow functions $k_{R,L}(x,t)$ -- right and left Fermi points respectively. The equations of motion are given by
\be
    \partial_{t}k_{R,L} +\varepsilon'(k_{R,L}) \partial_{x}k_{R,L} =0,
 \la{emlff}
\ee
which is an obvious consequence of the absence of interactions. Indeed, the derivative $\varepsilon'(k_{R,L})$ is the right (or left) Fermi velocity of particles, and  (\ref{emlff}) is nothing else but the statement that the momentum of a particle does not change in time. The classical action of 1D Fermi gas should reproduce (\ref{emlff}) as well as give the correct energy of the system $E=\int dx\,\int_{k_{L}(x)}^{k_{R}(x)}\frac{dk}{2\pi}\,\varepsilon(k)$.

We assume here that the dispersion of fermions is parity invariant $\epsilon(k)=\epsilon(-k)$ and consider the following Euclidian action
\be
 \la{aw}
    S = \int d^{2}x\, \left\{ \frac{i}{4\pi}\left[
    w\partial_{x}^{-1}\partial_{t}w
    -\bar w\partial_{x}^{-1}\partial_{t}\bar w \right]
    +\int_{-\bar w}^{w}\frac{dk}{2\pi}\, \varepsilon(k) \right\}.
\ee
Here $\varepsilon(k)$ is the dispersion (including chemical potential) of free fermions and $w,\bar w$ are independent variables which are Euclidian versions of $k_{R}$, $-k_{L}$. We identify the density of particles as $\rho = \frac{w+\bar w}{2\pi}$. The equations of motion corresponding to (\ref{aw})
\bea
    i\partial_{t}w+\partial_{x}\varepsilon(w) &=& 0,
 \nonumber \\
    -i\partial_{t}\bar w+\partial_{x}\varepsilon(\bar w) &=& 0
 \la{fmeq}
\eea
are, indeed, the Euclidian versions of (\ref{emlff}). Equations (\ref{fmeq}) are complex conjugates of each other ($\overline{\varepsilon(w)}=\varepsilon(\bar{w})$ as $\varepsilon(k)$ is a real function). The difference of these two equations give the continuity equation (\ref{continuity}) with the current $j=\frac{\varepsilon-\bar\varepsilon}{2\pi i}$. The path integral with the action (\ref{aw}) is the integral over two fields $w,\bar{w}$. We integrate out their difference $w-\bar{w}$ in a saddle point approximation. Namely, we re-write (\ref{aw}) in terms of combinations $w-\bar{w}$ and $w+\bar{w}$. Then, we take a variation of the action with respect to $w-\bar{w}$. This produces the continuity equation relating $w$ and $\bar{w}$. We solve the continuity equation introducing the displacement field.  Thus, we have $w$ and $\bar{w}$ in terms of $u$ as the saddle point trajectory. Namely,
\bea
    \rho &=& \frac{w+\bar w}{2\pi} = \rho_{0} +\partial_{x}u,
 \nonumber \\
    j &=& \frac{\varepsilon-\bar\varepsilon}{2\pi i} = -\partial_{t}u.
 \la{rjulf}
\eea
We substitute these expressions back into (\ref{aw}) and obtain
\be
 \la{awint}
    S[u] = \int d^{2}x\, \left\{ -\frac{1}{4\pi}(w-\bar{w})
    \left[\varepsilon(w)-\varepsilon(-\bar{w})\right]
    +\int_{-\bar w}^{w}\frac{dk}{2\pi}\, \varepsilon(k) \right\}.
\ee
We assume now that the integration variable of the path integral is the displacement field $u$. The fields $w,\bar{w}$ in (\ref{awint}) are not independent but are related to $u$ by (\ref{rjulf}). Deriving (\ref{awint}) we neglected the fluctuations around the saddle point as well as the changes in the measure of path integration. The corrections due to the neglected terms will be of the higher order in field gradients and are not essential for our calculation of the leading term of the EFP.

One can now use (\ref{awint}) in the path integral formulation of the quantum hydrodynamics (\ref{Z}) where the integration is taken over all configurations of the displacement field $u$. We note here that in the Galilean invariant systems the ``kinetic term'' of the hydrodynamic action (\ref{Shyd}) is fixed. The Lagrangian of the action (\ref{awint}) is a more complicated function of $\partial_{t}u$. In this case we derived it using the fact that fermions are free. In a more general problem of interacting particles the derivation of the hydrodynamic action requires the solution of the dynamic many body problem.

The Lagrangian of (\ref{awint}) is given by
\be
    L =-\frac{1}{4\pi}(w-\bar{w})
    \left[\varepsilon(w)-\varepsilon(-\bar{w})\right]
    +\int_{-\bar w}^{w}\frac{dk}{2\pi}\, \varepsilon(k).
 \la{lagrlf}
\ee
Now, we calculate the EFP for lattice fermions using the the Lagrangian (\ref{lagrlf}) with the Eq. (\ref{rjulf}), and the results of Appendix A. First, we calculate
\be
    dL =\frac{\varepsilon+\bar\varepsilon}{2}d\rho
    +\frac{w-\bar w}{2i}dj
\ee
and
\bea
    L_{j} &=& v = \frac{w-\bar w}{2i},
 \la{vlf} \\
    L_{\rho} &=& \frac{\varepsilon+\bar\varepsilon}{2},
 \\
    L_{jj} &=& \frac{2\pi}{\varepsilon'+\bar\varepsilon'},
 \\
    L_{\rho j} &=& -\frac{2\pi}{\varepsilon'+\bar\varepsilon'}
    \frac{\varepsilon'-\bar\varepsilon'}{2i},
 \\
    L_{\rho\rho} &=& \frac{2\pi}{\varepsilon'+\bar\varepsilon'}|\varepsilon'|^{2},
 \la{lrrlf}
\eea
where $\varepsilon'= \left|\frac{\partial\varepsilon}{\partial k}\right|_{k=w}$ and $\bar\varepsilon'= \left|\frac{\partial\varepsilon}{\partial k}\right|_{k=\bar w}$. In terms of the density and velocity
\be
    w=\pi \rho +iv.
 \la{wrvlf}
\ee
We emphasize that because of the absence of the Galilean invariance (the dispersion is  {\it not} $k^{2}/2m$), the current is {\it not} $\rho v$ but can be found from (\ref{rjulf},\ref{vlf}).

We obtain then an interesting relation
\be
     \kappa \equiv \sqrt{L_{\rho\rho}L_{jj}-L_{\rho j}^{2}}
     =\pi.
 \la{piid}
\ee
This relation can be considered as a special property of free fermions (with arbitrary dispersion!). Namely, one can trace the origin of (\ref{piid}) to the fact that each fermion occupies a fixed volume in the phase space. \footnote{For Calogero-Sutherland model (\ref{ercs}) we have $\kappa =\pi\lambda$. It means that the volume of the phase space per particle is changed by the factor of $\lambda$ which reflects the fractional statistics of particles.}


Let us now apply Riemann's trick to equations (\ref{fmeq}). Namely, we interchange independent and dependent variables so that $x=x(w,\bar w)$ and $t=t(w,\bar w)$. Then using (\ref{piid}, \ref{vlf}-\ref{lrrlf}) we re-write (\ref{fmeq}) as
%\be
%   -\frac{L_{\rho j}}{L_{jj}}
%    +i\sqrt{\frac{L_{\rho \rho}}{L_{jj}}-\left(\frac{L_{\rho j}}{L_{jj}}\right)^{2}}
%    =i\bar\varepsilon'
%\ee
\be
   \partial_{w}(x-i\bar\varepsilon' t) =0
 \la{fmeqR}
\ee
and its complex conjugate. The most general solution of (\ref{fmeqR}) is given implicitly by
\be
    w = F(z),
 \la{wfz}
\ee
where $F(z)$ is an arbitrary analytic function and
\be
    z = x +i\varepsilon'(w) t.
 \la{zw}
\ee
The equations (\ref{fmeqR}, \ref{zw}) reduce to equations for free continuous fermions if $\varepsilon(k)=k^{2}/2$.

Similarly to free continuous fermions, the EFP boundary conditions specify the form of the function $F(z)$ in (\ref{wfz}).
We define
\bea
    \tilde{w} &=& \frac{w-\pi\bar\rho}{2(1-\bar\rho)},
 \\
    \tilde{\theta} &=& \frac{\pi(\rho_{0}-\bar\rho)}{2(1-\bar\rho)},
\eea
where we assume lattice spacing to be 1 so that the maximal density of fermions on the lattice is $1$.
Then the EFP solution is given by $F(w)$ such that
\be
     \sin\tilde{w} = \sin\tilde{\theta}
     \frac{z}{\sqrt{z^{2}-R^{2}}}.
\ee
We immediately find at large distances ($z\to z_{0}=x+i\varepsilon_{0}' t \to \infty$)
\be
     w-\pi\rho_{0} \approx 2(1-\bar\rho)\frac{R^{2}}{2z_{0}^{2}}\tan\tilde{\theta}
\ee
and using (\ref{rvbosinf}) and (\ref{wrvlf}) we extract
\be
    \alpha = \frac{1}{2\pi}(1-\bar\rho)R^{2}\tan\tilde\theta.
\ee
We substitute this expression in (\ref{maingen}) and obtain
\be
    \partial_{\rho_{0}}S =2\pi(1-\bar\rho)R^{2}
    \tan\frac{\pi(\rho_{0}-\bar\rho)}{2(1-\bar\rho)},
\ee
so that
\be
 \la{dfpLat}
    S_{DFP} = -4(1-\bar\rho)^{2}R^{2}
    \ln\cos\frac{\pi(\rho_{0}-\bar\rho)}{2(1-\bar\rho)}.
\ee
In particular for $\bar\rho=0$ we obtain for the Emptiness Formation Probability
\be
 \la{efpLat}
    S_{EFP} = -4R^{2}
    \ln\cos\frac{\pi\rho_{0}}{2}
    = -4R^{2}
    \ln\cos\frac{k_{F}}{2}.
\ee
This result is the exact first term in $1/R$ expansion (\ref{exlf}). The next term is $\frac{1}{4}\ln R$.
It is interesting to note that as it should be, in the limit $\rho_{0}-\bar\rho\ll \rho_{0}$ the result (\ref{dfpLat}) reproduces the bosonization result (\ref{dfpbos}). Also, in the limit $\rho_{0},\bar\rho\ll 1$ the results (\ref{dfpLat},\ref{efpLat}) reproduce the corresponding results (\ref{dfpff},\ref{efpff}) for free continuous fermions.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Hydrodynamic approach to non-Galilean invariant systems}
\label{app_nGal}

The hydrodynamic description of Sec. \ref{sec_hydro} and the approach of Sec. \ref{sec_efp} can be easily generalized to non-Galilean invariant systems. We briefly list here relevant formulas leaving the details of (straightforward) calculations to the interested reader. We assume that a one-dimensional compressible liquid can be described by the partition function (\ref{Z}) where the functional integration is taken over all configurations of the displacement field $u$ which defines the hydrodynamic density and current by (\ref{displacement}) and where the Euclidian action (\ref{act}) can be written as
\be
    S = \int d^{2}x\, L(\rho,j).
 \la{actgen}
\ee
The Lagrangian density $L(\rho,j)$ is a function of $\rho$ and $j$. As in the main text we neglect the gradient corrections to the action (\ref{actgen}). In the case of non-Galilean invariant systems these gradient corrections will depend on gradients of current in addition to gradients of density. The case of Galilean invariant systems considered in the main text (\ref{Shyd}) can be obtained from the general one assuming the particular Galilean invariant form  of the Lagrangian $L(\rho,j) =j^{2}/2\rho +\rho\epsilon(\rho)$.

Variation of (\ref{actgen}) with respect to $u$ gives a generalized Euler equation which together with the continuity equation reads
\bea
    \partial_{t}\rho +\partial_{x}j &=& 0,
 \la{contgen} \\
    \partial_tL_j-\partial_x L_\rho  &=& 0,
 \la{eulergen}
\eea
where $L_{j}$ means $\partial L/\partial j$ etc.

If the deviation from the ground state is small, we can expand the action (\ref{actgen}) around $\rho=\rho_{0}$, $j=0$. We assume that $L_{\rho j}^{(0)}=0$, where superscript $(0)$ means that the derivative is calculated at the equilibrium values $\rho=\rho_{0}$ and $j=0$. We obtain for the action in harmonic approximation
\be
    S = \int d^{2}x\,\left[L_{jj}^{(0)}u_{t}^{2} +L_{\rho\rho}^{(0)}u_{x}^{2} \right].
\ee
We introduce a complex space-time coordinate
\bea
    z_{0} = x+iv_{s0}t,
 \la{z0gen}
\eea
where
\be
 \la{vs0}
    v_{s0} = \sqrt{\frac{L_{\rho \rho}^{(0)}}{L_{jj}^{(0)}}}
\ee
is the sound velocity at equilibrium. Let us define the coefficient $\alpha$ through the asymptotics of an EFP solution at $z_{0}\to\infty$ by (\ref{asymptu}). The asymptotics of the current and density are given by (\ref{rvbosinf}).

Our main formula (\ref{main}) for the variation of the EFP instanton action with respect to the background density becomes
\be
 \la{maingen}
    \partial_{\rho_{0}}S = 2\pi \kappa_{0}\,
    (\alpha+\bar\alpha),
\ee
where $\kappa_{0}$ is given by
\be
 \la{kappa0}
    \kappa_{0} =\sqrt{L_{\rho\rho}^{(0)}L_{jj}^{(0)}}.
\ee
The coefficient $\kappa_{0}$ is related to the compactification radius $R_{\rm comp}$ of bosons in the bosonization procedure  $\kappa_{0}=(2\pi R_{\rm comp})^{2}$. For free fermions $\kappa_{0}=\pi$ which corresponds to $R_{\rm comp}=1/\sqrt{4\pi}$.

